Conformal Graph Prediction with Z-Gromov-Wasserstein Distances

Supervised graph prediction addresses regression problems where the outputs are structured graphs. Although several approaches exist for graph-valued prediction, principled uncertainty quantification remains limited. We propose a conformal prediction framework for graph-valued outputs, providing distribution-free coverage guarantees in structured output spaces. Our method defines nonconformity via the Z-Gromov-Wasserstein distance, instantiated in practice through Fused Gromov-Wasserstein (FGW), enabling permutation invariant comparison between predicted and candidate graphs. To obtain adaptive prediction sets, we introduce Score Conformalized Quantile Regression (SCQR), an extension of Conformalized Quantile Regression (CQR) to handle complex output spaces such as graph-valued outputs. We evaluate the proposed approach on a synthetic task and a real problem of molecule identification.

==> final_paper/MetaboliteOld.tex <==

\begin{figure*}[t]
\centering

% -------------------- ROW 1 --------------------
\begin{minipage}{0.48\textwidth}
\centering
\textbf{Coloring — Conformal Prediction}

\vspace{4pt}

\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{images/main/colors/hist-adjacency-paul.pdf}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{images/main/colors/scatter-adjacency-paul.pdf}
\end{subfigure}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\centering
\textbf{Coloring — SCQR}

\vspace{4pt}

\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{images/main/colors/hist-adjacency-paul-scqr.pdf}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{images/main/colors/scatter-adjacency-paul-scqr.pdf}
\end{subfigure}
\end{minipage}

\vspace{0.8em}

% -------------------- ROW 2 --------------------
\begin{minipage}{0.48\textwidth}
\centering
\textbf{Metabolite Retrieval — Conformal Prediction}

\vspace{4pt}

\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{images/main/molecules/hist-laplacian-identity.pdf}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{images/main/molecules/scatter-laplacian-identity.pdf}
\end{subfigure}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\centering
\textbf{Metabolite Retrieval — SCQR}

\vspace{4pt}

\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{images/main/molecules/hist-laplacian-identity-scqr-embed.pdf}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{images/main/molecules/scatter-laplacian-identity-scqr-embed.pdf}
\end{subfigure}
\end{minipage}

\caption{
Conformal coverage and set size behavior across tasks.
Histograms show empirical coverage versus candidate set size.
Scatter plots show conformal set size versus candidate set size, the black dashed $y=x$ line indicates no reduction, and points below the line demonstrate cases where conformal filtering reduces the set.  Blue (resp. red) points indicate conformal sets containing the ground truth (resp. violations). For SCQR, the attribute function $\omega(x)$ is task-dependent:
$\omega(x)=|\mathcal{L}(x)|$ (candidate set size) for Coloring,
and $\omega(x)=\textsc{DreaMS}(x)$ (mass-spectrum embedding) for Metabolite.
}
\label{fig:cp_scqr_all}
\end{figure*}

\subsection{Results}
\paragraph{Coverage Validity and Efficiency.}  Across both tasks, empirical coverage remains close to the nominal $90\%$, confirming validity under $Z$-GW scoring, as reported in Table~\ref{tab:cp_scqr_comparison} and illustrated by the histograms in Figure~\ref{fig:cp_scqr_all}. 
We evaluate efficiency through conformal set size and reduction relative to the candidate library. On \textit{Coloring}, SCQR conditioned on $|\mathcal{L}(x)|$ performs similarly to CP: the median set size is $1$, with over $95\%$ average reduction. Conditioning brings limited additional benefit in this synthetic setting. On \textit{Metabolite Retrieval}, conditioning is crucial. SCQR based on $|\mathcal{L}(x)|$ does not improve efficiency. In contrast, conditioning on the spectral embedding $\textsc{DreaMS}(x)$ substantially reduces mean conformal set size from $24$ (CP) to $15$ while preserving coverage, increasing average reduction from $77.1\%$ to $84.8\%$. Figure~\ref{fig:cp_vs_scqr} shows that SCQR reduces heavy-tail behavior in conformal set sizes for metabolites.

\begin{table}
\centering
\small
\setlength{\tabcolsep}{3pt}
\caption{Results on metabolites with a $L$  and Id initialization}
\label{tab:zgw}
\begin{tabular}{lcccccc}
\toprule

& & \multicolumn{2}{c}{\makecell{\scriptsize \textbf{Conformal Set Size} $\downarrow$}}  & \multicolumn{2}{c}{\scriptsize \textbf{Reduction} \% $\uparrow$}\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} 
Z-GW
& \makecell{Emp.\\ Cov.}
& \makecell{Mean}
& \makecell{Med.}
& \makecell{Mean}
& \makecell{Med.}
& \makecell{Empty\\rate (\%) $\downarrow$} \\
\midrule

FNGW & $95.1\%$ & $44$ & $4$ & $63.8\%$ & $93.3\%$ & $0.0\%$ \\
FGW & $89.5\%$ & $15$ & $1$ &$84.8\%$ & $99.1\%$ & $0.4\%$ \\
GW & $95.0\%$ & $40$ & $3$ & $66.9\%$ & $94.4\%$ & $0.0\%$ \\
%W & $90.3\%$ & $163$ & $228$ & $0.9\%$ & $0.0\%$ & $8.8\%$ \\

\bottomrule
\end{tabular}
\end{table}



\paragraph{Versatility of $Z$-GW non-conformity scores.}
%@Thibualt ($\beta=0.4 \gamma=0.1$)
We illustrate the versatility of the $Z$-GW framework by comparing several instantiations. We fix the interpolation parameters: FGW ($\beta=0.5$) and FNGW ($\beta=\gamma=0.33$) . Pure GW, which only accounts for relational structure and ignores node features, naturally leads to higher uncertainty and larger candidate sets. In contrast, FGW reduces uncertainty by incorporating finer feature-level information in addition to structure, aligning with our expectations. For FNGW, performance depends more sensitively on the balance between structural, edge feature and node feature terms.

\paragraph{Top-$k$ vs Conformal.}
For a fair comparison, we calibrate SCQR ($\textsc{DreaMS}(x)$) so that its marginal coverage matches the top-5 accuracy of \textsc{SpecBridge} ($92.31\%$). 
Under this matched coverage level, the resulting conformal sets have mean size $33$ and median size $1$. 
Although half of the sets are singletons, the mean is inflated by a heavy tail. 
Among sets that contain the ground truth, $62.9\%$ have size $\leq 5$. 









==> final_paper/graph_prediction.tex <==
\subsection{Problem Setup}
\begin{figure}
    \centering
   \includegraphics[width=0.8\linewidth, trim=19 45 30 24, clip]{images/zgw.pdf}

    \caption{Z-GW distance}
    \label{fig:placeholder}
\end{figure}
\paragraph{Graphs as $Z$-networks.}
Graphs can be naturally viewed as finite $Z$-networks.
Let $G = (V,E,F)$ be a graph, where
$V$ is the node set with $|V| = n \in \mathbb{N}^*$,
$E \subseteq V \times V$ is the edge set, and
$F : V \to \mathbb{R}^d$ is a node feature map, with $F(i)$ denoting
the feature associated to node $i \in V$.
We associate to $G$ a $Z$-network $(V,\omega_G,\mu_G)$, where
$\mu_G \in \mathcal P(V)$ is a probability measure on $V$ (assumed uniform in this case), and
$\omega_G : V \times V \to \mathcal Z$ encodes pairwise relational
information between nodes.
This representation provides a unified way to encode both graph
structure and node attributes, enabling the comparison of graphs within
the general Z-GW distance.

In particular, the pairwise structure $\omega_G$ may combine structural
and node-level information as
\[
\omega_G(i,k)
=
\big(
\omega_G^{\mathrm{struct}}(i,k),
\; F_i
\big)
\in \mathcal Z := \Omega \times \mathbb{R}^d,
\]
where $\omega_G^{\mathrm{struct}} : V \times V \to \Omega$ encodes graph
connectivity (e.g., adjacency, shortest-path distance, or
Laplacian-based quantities), and $F_i \in \mathbb{R}^d$ denotes the feature
associated to node $i$. The product space $\mathcal Z$ is equipped with
a weighted $\ell_q$ metric
\[
d_{\mathcal Z}\big((a,u),(a',u')\big)
=
\Big(
(1-\alpha)\, d_\Omega(a,a')^q
+
\alpha d_{\mathbb R^d}(u,u')^q
\Big)^{1/q},\]
for  $\alpha \in [0,1],\; q \ge 1$. Additional technical details and further examples
are provided in Appendix~\ref{app:zgw_examples}.


\paragraph{Discrete $Z$-Gromov--Wasserstein for graphs.}
Let $G_1=(V_1,\omega_1,\mu_1)$ and $G_2=(V_2,\omega_2,\mu_2)$ be finite
graphs with $|V_1|=|V_2|=n$ and uniform measures.
The discrete $Z$-GW distance between $G_1$ and $G_2$ is defined as
\begin{equation}
    \min_{\pi\in\Pi(\mu_1,\mu_2)}
\left(
\sum_{i,k\in V_1}
\sum_{j,l\in V_2}
d_{\mathcal Z}\!\big(\omega_{1}(i,k),\omega_{2}(j,l)\big)^p
\,\pi_{ij}\pi_{kl}
\right)^{1/p}.
\end{equation}

In the finite graph setting with uniform measures, weak isomorphism admits
a simple characterization (see Proposition \ref{prop:weak_iso_perm} below). As a consequence, $\mathrm{GW}^Z_p$ defines a permutation-invariant
distance on graphs. 

\begin{proposition}[Weak isomorphism and permutation invariance]
\label{prop:weak_iso_perm}
Let $(V_1,\omega_1,\mu_1)$ and $(V_2,\omega_2,\mu_2)$ be finite
$Z$-networks associated to $G_1$ and $G_2$, respectively, with $|V_1|=|V_2|=n$ and uniform measures
$\mu_1=\mu_2$.
Then $G_1\sim G_2$ if and only if there exists a permutation matrix
$P\in\sigma_n$ such that $\omega_1 = P^\top\omega_2 P$.
\end{proposition}\begin{proof}
 Appendix \ref{proof:weak_iso_perm}. 
\end{proof}
From now on, we specialize the spaces $\mathfrak M$ and $\mathcal M$ to
graphs.
We denote by $\mathfrak M$ the collection of all graphs with at most $N$
nodes, i.e. $\mathfrak M = \bigsqcup_{n=1}^N
\mathcal{G}_n$, in which $\mathcal{G}_n$ are the space of all graphs with $n$ nodes represented in a labeled form, and by $\mathcal M$ the
corresponding quotient space where graphs are identified up to node
permutation.


\paragraph{Graph-valued prediction.}
We consider graph-valued prediction models \[
f_\theta:\mathcal X\to\mathfrak M
\] that map inputs
$x\in\mathcal X$ (e.g., spectra, images, or other descriptors)
to graph-valued outputs $y\in\mathfrak M$. In the remainder, we assume that these models have been learned on 
the training dataset $\{(X_i,Y_i)\}_{i=1}^n$ by minimizing a loss measuring discrepancy between predicted and
ground-truth graphs.
%predictor
%\[
%f_\theta:\mathcal X\to\mathfrak M
%\]
%by minimizing a loss measuring discrepancy between predicted and
%ground-truth graphs.
Crucially, such losses must be invariant to node relabeling; the
$\mathrm{GW}^Z_p$ distance satisfies this requirement by construction. In the experimental part, we consider two off-the-shelves graph prediction models $f_\theta$. One effectively relies on the minimization of a variant of FGW distance and leverages an encoder-decoder transformer architecture. Called Any2graph \citep{krzakala2024any2graph}, it is restricted to small-size graphs and will be used in the context of a synthetic dataset ("Coloring") that we slightly revisited. The other, named "SpecBridge" has been released very recently by \cite{wang2026specbridge} and is specialized on Metabolite identification from mass spectra. SpecBridge currently offers a significant improvement upon the state of the art by exploiting a mass spectra and metabolite autoencoders.
%//\FA{chosen to beis going to be a specific prediction model per molecular graphs.






==> source/SCQR.tex <==
\subsection{Locally Adaptive Graph Conformal Prediction}
\label{sec:scqr}

To address the challenge of providing distribution-free guarantees in complex, high-dimensional, or structured output spaces (such as graphs, manifolds, or functional data), we introduce Score Conformalized Quantile Regression (S-CQR). In such settings, performing traditional CQR directly on the output space $\mathcal{G}$ is often computationally or theoretically challenging. S-CQR circumvents this limitation by operating in the scalar nonconformity score
space, which remains well-defined regardless of the structure of the output.
By calibrating score thresholds instead of output coordinates, S-CQR provides
distribution-free guarantees for general complex output spaces while allowing
the induced candidate set size to adapt to input-dependent uncertainty.

\paragraph{Score Conformalized Quantile Regression}
Given a point predictor $f_\theta: \mathcal{X} \to \mathcal{G}$ and a nonconformity score $s(x, y) \in \mathbb{R}$, with $x\in\mathcal{X}$ and $y\in\mathcal{G}$. Graph conformal prediction as presented previously relies on a single global threshold, implicitly assuming homogeneous uncertainty across inputs—a one-size-fits-all assumption that is often violated in practice.


S-CQR relaxes this assumption by allowing the threshold to depend on input-dependent attributes $z(x)\in \mathcal{Z}$, which capture this heteroscedasticity. These attributes may be the input itself (identity map) or derived quantities reflecting its complexity.
In our metabolite identification setting, each input naturally comes with a finite candidate set of plausible molecular graphs. We therefore condition on the candidate set size $z(x)= |\mathcal{L}(x)|$, which already encodes information about task difficulty.

Concretely, we first train a quantile regression model $\psi: \mathcal{Z}\to \mathbb{R}$ using the pinball loss \PM{Wouldn't it be better to directly introduce the model here? Or do we wish to stay generec w.r.t. it?} to estimate $(1-\alpha)$-conditional quantile of $s(x,y)$ on  a training set. We again compute the adaptive residuals $E_i = s(X_i, Y_i) - \psi(z(X_i))$. We then compute the empirical quantile of the residuals: $\hat{q}_{1-\alpha} = \text{Quantile}\left(\{E_i\}_{i=1}^n, \frac{\lceil (n+1)(1-\alpha) \rceil}{n}\right)$. For a new input $X_{n+1}$, the conformal prediction set is:
 \begin{equation}
 \label{eq:scqr_set}
     \mathcal{C}(X_{n+1}) = \{ y \in \mathcal{G} : s(X_{n+1}, y) \le \psi(z(X_{n+1})) + \hat{q}_{1-\alpha}\}.
 \end{equation}

 The residuals $E_i$ may take both negative and positive values. Since $s(x,y)\ge 0$ and $s(x,y)=0$ indicates perfect conformity, negative residuals correspond to examples that are easier than predicted given $z(x)$, while positive residuals indicate an underestimation of difficulty. Retaining both is essential for adaptive and non-conservative conformal calibration.




\begin{proposition}[Marginal Coverage Guarantee of S-CQR]
\label{prop:scqr-validity}
Let $\{(X_i, Y_i)\}_{i=1}^{n+1}$ be exchangeable random variables, and let 
$z:\mathcal{X}\to\mathcal{Z}$ be a deterministic feature map.
Assume that the nonconformity score $s:\mathcal{X}\times\mathcal{G}\to\mathbb{R}$
and the quantile regression function $\psi:\mathcal{Z}\to\mathbb{R}$
are fixed measurable functions, independent of the calibration sample.
Then the S-CQR prediction set expressed in Eq. \ref{eq:scqr_set} satisfies
\begin{equation}
\mathbb{P}\!\left( Y_{n+1} \in \mathcal{C}(X_{n+1}) \right) \ge 1 - \alpha .
\end{equation}
\end{proposition}


\begin{proof}Let $E_i = s(X_i, Y_i) - \psi(z(X_i))$ be the meta-scores. By the exchangeability of the underlying data and the measurability of $s$, $z$ and $\psi$, the sequence $(E_1, \dots, E_{n+1})$ is exchangeable. The rank of $E_{n+1}$ is therefore uniform over $\{1, \dots, n+1\}$. Thus, $\mathbb{P}\!\left( E_{n+1} \le \hat q_{1-\alpha} \right)
\ge \frac{\lceil (n+1)(1-\alpha) \rceil}{n+1}
\ge 1 - \alpha$. Since $Y_{n+1} \in \mathcal{C}(X_{n+1}) \iff E_{n+1} \le \hat{q}$, the guarantee holds.\end{proof}

\begin{remark}[One-Sided Nature of S-CQR]Unlike the original CQR for real-valued regression which often produces two-sided intervals $[q_{low}, q_{high}]$, S-CQR is inherently one-sided. This is because nonconformity scores are typically designed to be non-negative, where smaller values represent better fits.\end{remark}

==> source/background.tex <==
\section{Background on Conformal Prediction}
Conformal Prediction (CP) provides finite-sample, distribution-free guarantees on the coverage of prediction sets.

\begin{definition}[Exchangeability]
A sequence of random variables $(Z_1, \dots, Z_{n+1})$ taking values in a measurable
space $\mathcal{Z}$ is said to be \emph{exchangeable} if, for any permutation
$\sigma$ of $\{1, \dots, n+1\}$ and for any $(z_1, \dots, z_{n+1}) \in \mathcal{Z}^{n+1}$, $
\mathbb{P}(Z_1 = z_1, \dots, Z_{n+1} = z_{n+1})
=
\mathbb{P}(Z_{\sigma(1)} = z_1, \dots, Z_{\sigma(n+1)} = z_{n+1}).
$
\end{definition}


In the regression setting, we observe exchangeable pairs $(X_i, Y_i)$ and have a pre-trained base predictor $f_\theta: \mathcal{X}\to\mathcal{Y}$. The framework relies on a \emph{nonconformity score} function $s: \mathcal{X \times \mathcal{Y}\to \mathbb{R}}$  that measures the discrepancy between the target $y$ and the prediction $f_\theta(x)$. For standard real-valued regression, a typical choice is the absolute residual:
\begin{equation}
s(x,y) = | y - f_\theta(x) |.
\end{equation}
Given a held-out calibration set $\mathcal{D}_{\text{cal}} = \{(X_i, Y_i)\}_{i=1}^n$, we compute the scores $R = \{R_1, \dots, R_n\}$ where $R_i = s(X_i, Y_i)$. We then compute the adjusted empirical quantile:
\begin{equation}
\hat{q}_{1-\alpha} = \text{Quantile}\left(\{R_i\}_{i=1}^n, \frac{\lceil (n+1)(1-\alpha) \rceil}{n}\right).
\end{equation}
For a new input $X_{n+1}$, the conformal prediction set is defined as:
\begin{equation}
\mathcal{C}(X_{n+1}) = \{ y \in \mathcal{Y} : s(X_{n+1}, y) \le \hat{q}_{1-\alpha} \}.
\end{equation}
By exchangeability of the calibration and test samples, the nonconformity scores
$\{R_i\}_{i=1}^{n+1}$ with $R_i = s(X_i, Y_i)$ form an exchangeable sequence.
Consequently, the rank of $R_{n+1}$ among $\{R_i\}_{i=1}^{n+1}$ is uniformly distributed,
which implies the marginal coverage guarantee \cite{vovk2005algorithmic}
\[
\mathbb{P}\big(Y_{n+1} \in \mathcal{C}(X_{n+1})\big) \ge 1 - \alpha,
\]
without any assumptions on the data distribution or the accuracy of the predictor.
We refer to \cite{angelopoulos2023conformal, shafer2008tutorial} for more details on conformal prediction.


\paragraph{Conformalized Quantile Regression}
To extend standard conformal prediction to better handle heteroscedasticity, Conformalized Quantile Regression (CQR) \cite{romano2019conformalized} improves the conformal framework by leveraging quantile regression \cite{koenker1978regression} to construct input-adaptive prediction intervals. Instead of relying on a fixed, globally calibrated residual, CQR employs two base models, $\hat{\psi}_{\alpha/2}(x)$ and $\hat{\psi}_{1-\alpha/2}(x)$, trained to estimate the lower and upper $(\alpha/2, 1-\alpha/2)$ quantiles of the conditional distribution $Y|X=x$. The nonconformity score is then defined as $s(x, y) = \max\{\hat{\psi}_{\alpha/2}(x) - y, y - \hat{\psi}_{1-\alpha/2}(x)\}$, which measures the signed distance of the target to the boundaries of the predicted interval. By computing the $(1-\alpha)$-th quantile of these scores, $\hat{q}_{1-\alpha}$, on a calibration set, the resulting prediction intervals $\mathcal{C}(x) = [\hat{\psi}_{\alpha/2}(x) - \hat{q}_{1-\alpha}, \hat{\psi}_{1-\alpha/2}(x) + \hat{q}_{1-\alpha}]$ achieve valid marginal coverage while dynamically adjusting their width to account for local uncertainty in the data. 

%Crucially, conformal prediction only requires:
%(i) a fixed predictor $f_\theta$ and
%(ii) a fixed score function $s$ used both on calibration and test data.
%In our setting, we will leverage this flexibility by letting $s$ be a graph-space distance induced by FGW.
\paragraph{Notation. } Let $\Sigma_n = \{ a \in \mathbb{R}^n_{+} :  \sum_{i=1}^n a_i = 1 \}$ be the probability simplex  and $\Pi(a,b)
=
\{
\pi \in \mathbb{R}_{+}^{n \times m}
\;:\;
\pi \mathbf{1}_m = a,\;
\pi^\top \mathbf{1}_n = b
\}$ be the set of  bistochastic matrices, where $\mathbf{1}_n \in \mathbb{R}^n$ is the all-ones vector with size $n$.  We denote $\sigma_n = \{P \in \{0,1\}^{n \times n}: P\mathbf{1}_n = \mathbf{1}_n,  P^\top\mathbf{1}_n = \mathbf{1}_n\}$ the set of permutation matrices. Calligraphic letters (e.g., $\mathcal{X}$) denote metric spaces. 
\subsection{Graph Supervised Prediction}

\paragraph{Graph space.}
Let $N \in \mathbb{N}*$ be the maximal number of nodes in the graphs we consider. We denote by $\mathcal{G}_n^{\mathrm{lab}}
\;=\;
\mathbb{R}^{n \times n} \times \mathbb{R}^{n \times d} \times \Sigma_n$ the space of labeled graphs, with a number of nodes up to $N$.
An element $y \in \mathcal{G}$ is represented as
\[
y = (A, F, a),
\]
where $n \leq N$ is the number of nodes, $A \in \mathbb{R}^{n \times n}$ encodes pairwise structure (e.g., adjacency, shortest path, or edge weights) between nodes, $F \in \mathbb{R}^{n \times d}$ is the node feature matrix, and $a \in \Sigma_n$ is a probability vector over nodes, which is set to be the uniform over $\{1,\dots,n\}$.

\paragraph{Graph Isomorphism} 
Graphs are defined up to node permutations: two graph triplets $y=(A,F,a)$ and $y'=(A',F',a')$ are said to be isomorphic $y\cong y'$ if there exists a permutation matrix $P\in \sigma_n$ such that 
$(A',F',a') = (PAP^\top,\; PF,\; Pa)$.
Such a permutation corresponds to a relabeling of the nodes and leaves the underlying graph unchanged. 

\paragraph{Quotient Space.}

The space $\mathcal{G}_n^{\mathrm{lab}}$ is acted upon by the permutation group $\sigma_n$ through $P\cdot y = (P A P^\top,\; P F,\; P a)$, for some $P\in \sigma_n$. The corresponding quotient $\mathcal{G}_n
\;=\;
\mathcal{G}_n^{\mathrm{lab}} \big/ \sigma_n$
identifies graph representations that differ only by a permutation of nodes. 
For a graph $y \in \mathcal{G}_n^{\mathrm{lab}}$, we denote by $[y] := \{\, P \cdot y \;:\; P \in \sigma_n \,\}$
the associated equivalence class under node permutations; by construction, $[y] \in \mathcal{G}_n$.
Since graphs with different numbers of nodes belong to ambient spaces of different dimensions and are associated with distinct permutation groups, they cannot be identified through relabeling. The overall space of graphs is therefore given by the disjoint union of these quotient spaces,
\[
\mathcal{G}
\;=\;
\bigsqcup_{n=1}^N
\mathcal{G}_n
\;=\;
\bigsqcup_{n=1}^N
\big( \mathbb{R}^{n \times n} \times \mathbb{R}^{n \times d} \times \Sigma_n \big) \big/ \sigma_n.
\]
An element of $\mathcal{G}$ thus represents an equivalence class of labeled graph triplets under node permutations, corresponding to an unlabeled graph with node features and weights.

We consider a supervised learning setting where inputs $x$ lie in some space $\mathcal{X}$ (e.g., spectra, images, or other descriptors) and outputs are graphs $y \in \mathcal{G}$.
Given training data $\{(x_i,y_i)\}_{i=1}^n$, the goal is to learn a predictor
\[
f_\theta : \mathcal{X} \to \mathcal{G},
\]
that minimizes a suitable graph-valued loss.
To compare graphs, we equip $\mathcal{G}$ with a distance between predictions and ground-truth outputs.

\paragraph{Fused Gromov--Wasserstein.}
A natural way to compare graphs while being invariant to node permutations is the fused Gromov--Wasserstein (FGW) discrepancy \cite{vayer2020fused}.
Given two graphs
\[
y = (A,F,a) 
\quad\text{and}\quad
y' = (A',F',b),
\]
FGW extends the classical Gromov--Wasserstein (GW) discrepancy \cite{memoli2011gromov} by augmenting the structure-matching term between pairwise relations with an additional feature-matching term between node attributes. The term fused reflects the fact that feature similarity and structural similarity are jointly accounted for within a single optimal transport problem through a common coupling.



Let $\mathcal{L}_{\text{feat}}$ and $\mathcal{L}_{\text{struc}}$ be non-negative loss functions on node features and structural entries, respectively.
The  FGW objective between $y$ and $y'$ is
\begin{align}
\label{eq:fgw}
\mathrm{FGW}_\lambda^2(y,y')
=
\min_{\pi\in \Pi(a,b)}
(1 - \lambda)\sum_{i,k} \mathcal{L}_{\text{feat}}&(F_i, F'_k)\, \pi_{ik}\notag\\
+
\lambda \underbrace{\sum_{i,j,k,\ell} \mathcal{L}_{\text{struc}}(A_{ij}, A'_{k\ell})\, \pi_{ik} \pi_{j\ell}}_{\text{Gromov-Wasserstein term}}
,
\end{align}
where $\Pi(a,b)$ is the set of couplings with marginals $a$ and $b$, $\lambda \ge 0$ balances features and structure. In practice, $\mathcal{L}_{\text{feat}}$ and $\mathcal{L}_{\text{struc}}$ are typically chosen as squared Euclidean losses, e.g.,
$\mathcal{L}_{\text{feat}}(F_i,F'_k) = \lVert F_i - F'_k\rVert_{\mathbb{R}^d}^2$ \PM{Could you name the matrix norm?}and
$\mathcal{L}_{\text{struc}}(A_{ij},A'_{k\ell}) = (A_{ij} - A'_{k\ell})^2$.


The optimal coupling $P^\star$ can be interpreted as a (soft) node matching, and \eqref{eq:fgw} defines a permutation-invariant discrepancy on $\mathcal{G}$.
In the following, we use $\mathrm{FGW}^2_\lambda(y,y')$ as the underlying pseudo-metric on the graph space. 
\begin{remark}[Relevance to Molecular Chemistry]
The FGW framework is particularly well-suited for molecular applications as it explicitly models the dual nature of chemical entities: the connectivity of the molecular scaffold ($A$) and the chemical identity of individual atoms ($F$).  This approach aligns with recent work in graph-based molecular modeling, where FGW-type objectives serve as the central training loss, including barycenter methods for graph-valued regression \cite{brogat2022learning,yang2024exploiting}, linear graph-valued regression \cite{calissano2022graph},deep end-to-end graph-valued regression \cite{shit2022relationformer, krzakala2024any2graph}, and graph-level auto-encoders \cite{krzakala2025quest}.
\end{remark}

\subsection{Conformal Prediction}

\begin{definition}[Exchangeability]
A sequence of random variables $(Z_1, \dots, Z_{n+1})$ taking values in a measurable
space $\mathcal{Z}$ is said to be \emph{exchangeable} if, for any permutation
$\sigma$ of $\{1, \dots, n+1\}$ and for any $(z_1, \dots, z_{n+1}) \in \mathcal{Z}^{n+1}$, $
\mathbb{P}(Z_1 = z_1, \dots, Z_{n+1} = z_{n+1})
=
\mathbb{P}(Z_{\sigma(1)} = z_1, \dots, Z_{\sigma(n+1)} = z_{n+1}).
$
\end{definition}

Conformal Prediction (CP) provides finite-sample, distribution-free guarantees on the coverage of prediction sets.
In the regression setting, we observe exchangeable pairs $(X_i, Y_i)$ and have a pre-trained base predictor $f_\theta: \mathcal{X}\to\mathcal{Y}$. The framework relies on a \emph{nonconformity score} function $s: \mathcal{X \times \mathcal{Y}\to \mathbb{R}}$  that measures the discrepancy between the target $y$ and the prediction $f_\theta(x)$. For standard real-valued regression, a typical choice is the absolute residual:
\begin{equation}
s(x,y) = | y - f_\theta(x) |.
\end{equation}
Given a held-out calibration set $\mathcal{D}_{\text{cal}} = \{(X_i, Y_i)\}_{i=1}^n$, we compute the scores $R = \{R_1, \dots, R_n\}$ where $R_i = s(X_i, Y_i)$. We then compute the adjusted empirical quantile:
\begin{equation}
\hat{q}_{1-\alpha} = \text{Quantile}\left(\{R_i\}_{i=1}^n, \frac{\lceil (n+1)(1-\alpha) \rceil}{n}\right).
\end{equation}
For a new input $X_{n+1}$, the conformal prediction set is defined as:
\begin{equation}
\mathcal{C}(X_{n+1}) = \{ y \in \mathcal{Y} : s(X_{n+1}, y) \le \hat{q}_{1-\alpha} \}.
\end{equation}
By exchangeability of the calibration and test samples, the nonconformity scores
$\{R_i\}_{i=1}^{n+1}$ with $R_i = s(X_i, Y_i)$ form an exchangeable sequence.
Consequently, the rank of $R_{n+1}$ among $\{R_i\}_{i=1}^{n+1}$ is uniformly distributed,
which implies the marginal coverage guarantee \cite{vovk2005algorithmic}
\[
\mathbb{P}\big(Y_{n+1} \in \mathcal{C}(X_{n+1})\big) \ge 1 - \alpha,
\]
without any assumptions on the data distribution or the accuracy of the predictor.
We refer to \cite{angelopoulos2023conformal, shafer2008tutorial} for more details on conformal prediction.


\paragraph{Conformalized Quantile Regression}
To extend standard conformal prediction to better handle heteroscedasticity, Conformalized Quantile Regression (CQR) \cite{romano2019conformalized} improves the conformal framework by leveraging quantile regression \cite{koenker1978regression} to construct input-adaptive prediction intervals. Instead of relying on a fixed, globally calibrated residual, CQR employs two base models, $\hat{\psi}_{\alpha/2}(x)$ and $\hat{\psi}_{1-\alpha/2}(x)$, trained to estimate the lower and upper $(\alpha/2, 1-\alpha/2)$ quantiles of the conditional distribution $Y|X=x$. The nonconformity score is then defined as $s(x, y) = \max\{\hat{\psi}_{\alpha/2}(x) - y, y - \hat{\psi}_{1-\alpha/2}(x)\}$, which measures the signed distance of the target to the boundaries of the predicted interval. By computing the $(1-\alpha)$-th quantile of these scores, $\hat{q}_{1-\alpha}$, on a calibration set, the resulting prediction intervals $\mathcal{C}(x) = [\hat{\psi}_{\alpha/2}(x) - \hat{q}_{1-\alpha}, \hat{\psi}_{1-\alpha/2}(x) + \hat{q}_{1-\alpha}]$ achieve valid marginal coverage while dynamically adjusting their width to account for local uncertainty in the data. 

%Crucially, conformal prediction only requires:
%(i) a fixed predictor $f_\theta$ and
%(ii) a fixed score function $s$ used both on calibration and test data.
%In our setting, we will leverage this flexibility by letting $s$ be a graph-space distance induced by FGW.


==> source/conclusion.tex <==
\section{Conclusion and Future Directions}

\GM{Multivariate settings for the score, amortization on the computation of FGW for faster computations. }

\section*{Impact Statement}
This paper presents work whose goal is to advance the field of machine learning. There are many potential societal consequences of our work, none of which we feel must be specifically highlighted here.

==> source/conformalgraph.tex <==
\newcommand{\G}{\mathcal{G}}
\newcommand{\Giso}{\G/\!\cong}
\newcommand{\dGW}{d_{\mathrm{GW}}}
\newcommand{\dFGW}{d_{\mathrm{FGW}}}
\newcommand{\dfGW}

\section{Conformal Graph Prediction}
\label{sec:cgp}

We now adapt conformal prediction to the setting where outputs are graphs $y \in \mathcal{G}$.
 We retain the supervised setup introduced above and assume a
trained predictor
$f_\theta : \mathcal{X} \to \mathcal{G}$, yielding a point prediction
$\hat y = f_\theta(x)$. 

\begin{assumption}
    The data consist of pairs $(X_i, Y_i) \in \mathcal{X} \times \mathcal{G}$, which are exchangeable.
\end{assumption}

\PM{Simple, but I would write why this assumption is needed.}

\paragraph{Graph-based nonconformity scores.}
Given a graph dissimilarity $d : \mathcal{G} \times \mathcal{G} \to
\mathbb{R}_{\ge 0}$, we define the nonconformity score 
\begin{equation}
\label{eq:score-graph}
s(x,y) = d\big(f_\theta(x), y\big).
\end{equation}
In this work, we propose to use the FGW as the graph non-similarity score. More precisely, we adopt
\begin{equation}
    s(x,y) = d_{\mathrm{FGW}}(f_\theta(x), y)) := \mathrm{FGW}_\lambda^2(f_\theta(x), y).
\end{equation}

\begin{proposition}[Validity of GW/FGW-based nonconformity scores]
\label{prop:validity-fgw}
Let $\G$ denote the space of finite attributed graphs, and let $\Giso$ be the quotient space of graph isomorphism classes. The  $d_\mathrm{GW}$ and its fused variant $d_\mathrm{FGW}$ define Borel-measurable functions on $(\Giso) \times (\Giso)$. 

Consequently, the nonconformity score 
\begin{equation}
    s(x,y) := d_\mathrm{(F)GW}(f_\theta(x), y)
\end{equation}
is measurable and permutation invariant. If the data $(X_i, Y_i)_{i=1}^n$ are exchangeable, then the induced sequence of scores $\{s(X_i, Y_i)\}_{i=1}^n$ is also exchangeable.
\end{proposition}

\begin{proof}\FA{That proposition is not proved: be careful that Gromov-Wasserstein distance is defined over the space of metric-measured spaces. I would first consider the continuous case of mmd, and the the discrete case. I will come back to \cite{memoli2011gromov}}.
Both GW and FGW distances are formulated as optimal transport problems over compact metric-measure spaces and depend strictly on the isomorphism classes of the graphs. Their objective functions are continuous with respect to the underlying cost matrices, which implies Borel measurability on the quotient space $\Giso$. Since both discrepancies are invariant under node relabelings (isomorphisms), the resulting score function $s$ is permutation invariant. By the property of measurable functions of exchangeable random variables, the exchangeability of the input data sequence $(X_i, Y_i)$ directly transfers to the sequence of nonconformity scores.
\PM{You can't write it more formally?}
\PM{Citation to every statement?}
\end{proof}


\begin{lemma}
\label{lemma:invariant_score}
    Let $s(x,y) = d_{\mathrm{FGW}}(f_\theta(x), y)$, then $s(x, y) = s(x, P \cdot y)$ for all $P \in \sigma_n$ and$ (x,y)\in \mathcal{X} \times \mathcal{G}_n^{\mathrm{lab}}$, where $P \cdot y = (PAP^\top, PF, Pa).$
\end{lemma}
\begin{proof}
Fix $x$ and let $y = (A,F,a) \in \mathcal{G}_n^{\mathrm{lab}}$ be a graph with $n$ nodes.
The FGW discrepancy between $f_\theta(x)$ and $y$ is defined as
\[
d_{\mathrm{FGW}}(f_\theta(x), y)
=
\min_{\pi \in \Pi(a,\hat a)}
(1-\lambda)\langle C_F, \pi \rangle
+
\lambda \langle C_A, \pi \otimes \pi \rangle,
\]
where $C_F$ and $C_A$ denote the feature and structure cost tensors, respectively. \GM{Finish}
\end{proof}

Similar to the classical case, we compute empirical
$(1-\alpha)$-quantile $\hat q_{1-\alpha}$ using the the calibration scores
$R_i = s(X_i,Y_i)$. The conformal graph prediction set for
a new input $X_{n+1}$ is then given by
\begin{equation}
\label{eq:fgw-ball}
\mathcal{C}(X_{n+1})
=
\Big\{
y \in \mathcal{G} :
d_\mathrm{FGW}\big(f_\theta(X_{n+1}), y\big) \le \hat q_{1-\alpha}
\Big\},
\end{equation}leading to the desired coverage guarantee $\mathbb{P}\big( Y_{n+1} \in \mathcal{C}(X_{n+1}) \big) \ge 1-\alpha$. 

\begin{remark}[Representation vs. Exchangeability]
\FA{there must be a discussion about exchangeability, because indeed the node permutation invariance raises a difficulty but it should not be here. That's tough I think.}
\GM{Either re-write or remove it}
In the context of conformal prediction, it is often assumed \PM{Citations?} that any measurable score function preserves exchangeability. However, for graph-valued data, one must distinguish between the isomorphism class $[g] \in \Giso$ and its representation as an adjacency matrix $A$. If a score $s$ is not permutation invariant, it is not a well-defined function on $\Giso$, but rather a function of the specific node ordering. Unless these orderings are themselves sampled exchangeably, the resulting score sequence may violate the exchangeability requirement. By using the (F)GW distance, which is invariant by construction, we ensure the score is a function of the isomorphism class, thus preserving the validity of the conformal guarantee.
\PM{Really sorry, I absolutely did not understand this paragraph.}
\end{remark}

In practice, $\mathcal{G}$ is an infinite dimensional space \FA{Be careful: we must be very clear when we talk about relaxed graphs, continuous node labems etc..} and \eqref{eq:fgw-ball} is defined implicitly.
We therefore approximate $\mathcal{C}(X_{n+1})$ by intersecting the FGW-ball with a finite candidate set. 

\paragraph{Implicit Sets and Intersection with Candidates.}

The conformal set defined in \eqref{eq:fgw-ball} is an implicit subset of the graph space $\mathcal{G}$, specified through a membership predicate rather than explicit enumeration. For any candidate graph $y \in \mathcal{G}$, membership is determined by evaluating the nonconformity score $s(x,y)$ and comparing it to the calibrated threshold. In molecular graph domains, however, $\mathcal{G}$ is combinatorially large, making the explicit materialization of $\mathcal{C}(x)$ computationally infeasible.

To obtain a finite and tractable prediction set, we intersect the implicit conformal set with an input-dependent candidate library $\mathcal{L}(x) \subset \mathcal{G}$ (e.g., a metabolite database determined by a mass spectrum):
\begin{equation}
\label{eq:candidate}
\mathcal{C}_{\mathcal{L}}(x) = \mathcal{C}(x) \cap \mathcal{L}(x) = \{y \in \mathcal{L}(x) : s(x, y) \leq \hat{q}_{1-\alpha}\}.
\end{equation}
In identification tasks, the candidate library is typically constructed to be complete, in the sense that the ground-truth output is contained almost surely, i.e., $\mathbb{P}(Y_{n+1} \in \mathcal{L}(X_{n+1} )) = 1$.
Under this assumption, $\mathcal{C}_{\mathcal{L}}(x)$ coincides with the exact conformal prediction set restricted to the reduced output space $\mathcal{L}(x)$ and therefore inherits the marginal coverage guarantee.

In practice, candidate libraries are often restricted to graphs of fixed size, i.e.,
$\mathcal{L}(x) \subset \mathcal{G}_n^{\mathrm{lab}}$.
The following proposition shows that, when using a permutation-invariant score, this restriction admits a canonical interpretation on the quotient space of unlabeled graphs and does not affect the validity of conformal prediction on the full graph space $\mathcal{G}$.



\begin{proposition}
\label{prop:equi}
Let $s(x,y) = d_{\mathrm{FGW}}(f_\theta(x), y)$ be a nonconformity score and let
$\mathcal{L}(x) \subset \mathcal{G}_n^{\mathrm{lab}}$ be a finite candidate set \FA{of graphs of the same size $n$}.
Then the conformal prediction set $\mathcal{C}_{\mathcal{L}}(x)$ admits a canonical representation as a subset of the quotient space $\mathcal{G}_n = \mathcal{G}_n^{\mathrm{lab}} / \sigma_n$.
\end{proposition}
\begin{proof}
By Lemma~\ref{lemma:invariant_score}, $s(x, y) = s(x, P \cdot y)$ for all $P \in \sigma_n$.
Hence, for any graph $y \in \mathcal{L}(x)\subset\mathcal{G}_n^{\mathrm{lab}}$, all elements of its equivalence class
$[y] = \{ P \cdot y : P \in \sigma_n \}$ share the same score value. Since $\mathcal{L}(x) \subset \mathcal{G}_n^{\mathrm{lab}}$ may contain multiple labeled representations corresponding to the same equivalence class, the conformal selection rule given by Eq.~\ref{eq:candidate}
either includes all elements of $[y]$ or excludes all of them.
Thus, by retaining a single representative per equivalence class—e.g., any canonical representative—the conformal prediction set can be identified with a set of equivalence classes $[y] \in \mathcal{G}_n$.
This yields a canonical representation of $\mathcal{C}_{\mathcal{L}}(x)$ as a subset of the quotient space $\mathcal{G}_n \subset \mathcal{G}$.
\end{proof}

\begin{remark}The restriction to a candidate library preserves the finite-sample marginal coverage
guarantee provided that the exchangeability assumption between calibration and test data
holds. If the ground-truth output $Y_{n+1}$ may lie outside $\mathcal{L}(X)$, the coverage
degrades according to the probability of library incompleteness: $
\mathbb{P}(Y_{n+1}  \in \mathcal{C}_{\mathcal{L}}(X_{n+1} ))
\;\geq\;
(1 - \alpha) - \mathbb{P}(Y_{n+1}  \notin \mathcal{L}(X_{n+1} ))$.
\end{remark}

In practical identification problems, each input $x$ is naturally associated with a finite candidate library $\mathcal{L}(x) \subset \mathcal{G}$ of plausible outputs, whose size may vary significantly between inputs. This variability is not incidental: larger candidate sets typically correspond to more ambiguous or difficult instances, while smaller candidate sets indicate stronger prior constraints and easier identification problems. As a result, the cardinality $|\mathcal{L}(x)|$ provides an input-dependet proxy for heteroscedastic uncertainty. Exploiting this information is crucial to avoid overly conservative conformal sets for easy inputs and undercoverage for hard ones.








==> source/experiments.tex <==
\section{Numerical Experiments}

\begin{table*}[t]
\centering
\caption{Comparison of conformal prediction (CP) and score-conditional quantile regression (SCQR) on graph-valued outputs with finite candidate sets on Coloring dataset. Both methods are evaluated at nominal coverage level $1-\alpha$, with $\alpha=0.1$. Arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) values are preferable.}
\label{tab:cp_scqr_comparison}
\begin{tabular}{llcccccc}
\toprule
Z-GW distance
& Method 
& \makecell{Empirical \\ Coverage}
& \makecell{Mean\\set size $\downarrow$}
& \makecell{Median\\set size $\downarrow$}
& \makecell{Mean\\reduction (\%) $\uparrow$}
& \makecell{Median\\reduction (\%) $\uparrow$}
& \makecell{Empty\\rate (\%) $\downarrow$} \\
\midrule
\multirow{2}{*}{FGW - Adj}
& CP   & $0.90$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ \\
& SCQR & $0.90$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ \\
\midrule
\multirow{2}{*}{FGW - SP}
& CP   & $0.90$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ \\
& SCQR & $0.90$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ \\
\midrule
\multirow{2}{*}{FGW - Laplacian}
& CP   & $0.90$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ \\
& SCQR & $0.90$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ \\
\midrule
\multirow{2}{*}{FGW - Diffused}
& CP   & $0.90$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ \\
& SCQR & $0.90$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ & $\,\cdot\,$ \\
\bottomrule
\end{tabular}
\end{table*}







\GM{\cite{calissano2024conformal} check if we can compare} 
\subsection{Synthetic Coloring Dataset}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/cov.pdf}
        \caption{}
        \label{fig:sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/scatter.pdf}
        \caption{}
        \label{fig:sub2}
    \end{subfigure}

    \caption{(a) Conformal coverage rate as a function of candidate set size, computed by binning candidate sizes and plotting the fraction of samples in each bin whose conformal set contains the ground-truth graph; the dashed horizontal line denotes the target coverage level. (b) Scatter plot of conformal set size versus candidate set size; the red dashed $y=x$ line indicates no reduction, and points below the line show cases where conformal filtering reduces the set. Blue points indicate conformal sets containing the ground truth; red points indicate violations.}
    \label{fig:main}
\end{figure*}


The Coloring dataset \cite{krzakala2024any2graph} consists of pairs $(x, y)$, where $x$ is an image encoding a combinatorial graph coloring instance and $y$ is its ground-truth graph representation. Nodes are associated with discrete colors, and edges encode the specific constraints of the coloring problem. The learning task is to recover the underlying graph structure from the visual observation, serving as a controlled benchmark for image-to-graph inference with structured node attributes.

\textbf{Metabolite-Style Candidate Sets.} To emulate the candidate-based setting of metabolite identification, we adapt this benchmark by constructing a restricted candidate set $\mathcal{L}(x)$ for each test instance. For a given pair $(x, y)$, we scan the test split and retain all graphs with identical node-type configurations (i.e., matching histograms of node attributes). This simulates a realistic identification scenario where the candidate library contains multiple structural isomers or topologically similar graphs, and the model must identify the correct structure among them.

\textbf{Model and Training.} We employ the \textsc{Any2Graph} architecture \cite{krzakala2024any2graph} as our graph regressor $f_\theta$. The model is trained to map images directly to the space of graphs by minimizing the Partially Masked Fused Gromov--Wasserstein (PMFGW) loss. This ensures that the model outputs are optimized for the same metric space used in our nonconformity scoring. 

\textbf{Experimental Protocol.} We partition the dataset into 100k samples for training, 10k for calibration (validation), and 10k for testing. Following the theory in Section \ref{sec:cgp}, we compute the calibration scores $\{s_i\}_{i=1}^{10,000}$ using the FGW distance. For standard CP with a fixed quantile, the entire calibration set is used to estimate the quantile threshold. In contrast, for S-CQR, the calibration set is split into two equal parts: one half is used to train the quantile regression model that maps candidate set size to score $1-\alpha$-quantiles, while the other half is used to compute the empirical quantile of the resulting residual scores. 

\paragraph{Results.}
Using the entire test split, we assess empirical coverage by verifying whether the ground-truth output belongs to the corresponding conformal prediction set. In addition, we report the median and mean reduction in prediction set size relative to the original candidate set of plausible graphs. The results are summarized in Table~\ref{tab:scqr_comparison}.

Size reduction is computed per test instance as 
$\frac{|\mathcal{L}(x)| - |\mathcal{C}(x)|}{|\mathcal{L}(x)|} \times 100\%$. We report two aggregates: the median reduction (robust ‘typical’ shrinkage across instances) and the mean reduction (sensitive to the tail of very large shrinkages). A large gap between mean and median indicates a skewed distribution where most instances shrink little, but a minority shrink a lot. For CP, the median reduction is small, indicating most test instances are only slightly reduced; however, the mean reduction is much larger, implying a minority of instances experience substantial shrinkage. S‑CQR yields larger typical reductions and a higher mean reduction.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/scores_vs_candidate_size_both_test.pdf}
    \caption{Gray points show non‑conformity scores between the model prediction and the ground‑truth candidate. The fixed black dashed line is the standard CP threshold. Solid blue/green lines are SCQR thresholds (MLP/RF) with the conformal offset $\hat q_{1-\alpha}$; the lighter dashed lines show the corresponding base regressors without the offset.}
    \label{fig:threshold}
\end{figure}







==> source/higherorder.tex <==
\section{Higher-Order Graphs Distances for Tighter Conformal Sets}

\FA{not sure this is the right definition}. \FA{ Denote $\exp(-\lambda L)_n= \sum_{i=1}^n (-\lambda)^{i}\frac{L^{i}}{i!}$. Let us move to $FGW_{n,\lambda}(y,y')= FGW(exp(-\lambda L)_n, F, exp(-\lambda L')_n, F'$.}

We consider refining conformal prediction in graph spaces by incorporating
higher-order structural information via powers of the adjacency matrix. Recall that $y = (A,F)$ denotes a finite attributed graph with adjacency $A$ and node features $F$.

\paragraph{Higher-order graph representations.}
For $k \ge 1$, we define the $k$-hop graph representation $y^{(k)} := (A^k, F)$, where $A^k$ encodes walk-based connectivity. 
We define the corresponding $k$-hop FGW 
\begin{equation}
    {\mathrm{FGW}}^{(k)}(y,g)
:= {\mathrm{FGW}}\big(y^{(k)}, g^{(k)}\big).
\end{equation}
and the associated
$s_k(x,y) := {\mathrm{FGW}}^{(k)}\big(f_\theta(x), y\big)$. 

By permutation invariance and measurability of FGW, the scores ${\mathrm{FGW}}^{(k)}$ are
well-defined and exchangeable under the same assumptions as in
Section~\ref{sec:cgp}, yielding distribution-free conformal validity.
\GM{ Maybe we can do something to prove some tighter average conformal set size }




==> source/metabolite_exp.tex <==
\subsection{Metabolite identification}

We consider a metabolite identification task where the goal is to recover the molecular structure of a small molecule from its tandem mass (MS/MS) spectrum.
Each input $x$ is a spectrum and each output $y$ is a molecular graph.
For every spectrum $x$, we assume access to a finite candidate set $\mathcal{L}(x) \subset \mathcal{G}$ of plausible molecular structures (e.g., retrieved from a spectral library), and the learning problem consists in selecting or ranking candidates.



==> source/theory.tex <==
\section{Z-Gromov-Wasserstein}

\begin{definition}[Metric Measure Spaces]
    A metric measure space (mm-space) is defined as triple $(\mathcal{X}, d_\mathcal{X}, \mu_\mathcal{X})$, where $ (\mathcal{X}, d_\mathcal{X})$ is a compact metric space and $\mu_\mathcal{X}$ is a Borel probability measure on $\mathcal{X}$ with $\mu_\mathcal{X}(\mathcal{X})=1$ and full support, $\mathrm{supp}(\mu_\mathcal{X}) = \mathcal{X}$.
\end{definition}


\begin{definition}[Isomorphism of Metric Measure Spaces]
Two metric measure spaces $(\mathcal{X}, d_\mathcal{X}, \mu_\mathcal{X})$ and
$(\mathcal{Y}, d_\mathcal{Y}, \mu_\mathcal{Y})$ are said to be \emph{isomorphic} if there
exists an isometry $\psi : \mathcal{X} \to \mathcal{Y}$ such that the pushforward measure
satisfies $\psi_{\#}\mu_\mathcal{X} = \mu_\mathcal{Y}$.
We write $(\mathcal{X}, d_\mathcal{X}, \mu_\mathcal{X}) \cong
(\mathcal{Y}, d_\mathcal{Y}, \mu_\mathcal{Y})$to denote this equivalence.
\end{definition}

\begin{definition}[Weak isomorphism of $Z$-networks]
Let $X=(\mathcal{X},\omega_\mathcal{X},\mu_\mathcal{X})$ and
$Y=(\mathcal{Y},\omega_\mathcal{Y},\mu_\mathcal{Y})$ be $Z$-networks.
We say that $X$ and $Y$ are \emph{weakly isomorphic} if there exists a third
$Z$-network $(\mathcal{W},\omega_\mathcal{W},\mu_\mathcal{W})$ together with
measure-preserving maps
\[
\phi_\mathcal{X}:\mathcal{W}\to\mathcal{X},
\qquad
\phi_\mathcal{Y}:\mathcal{W}\to\mathcal{Y},
\]
such that
\[
\omega_\mathcal{W}
=
\phi_\mathcal{X}^\ast \omega_\mathcal{X}
=
\phi_\mathcal{Y}^\ast \omega_\mathcal{Y}
\quad
\mu_\mathcal{W}\otimes\mu_\mathcal{W}\text{-a.e.}
\]
We write $X\sim Y$ to denote weak isomorphism.
\end{definition}

\paragraph{Gromov-Wasserstein }
Given two metric measure spaces $(\mathcal{X}, d_\mathcal{X}, \mu_\mathcal{X})$ and
$(\mathcal{Y}, d_\mathcal{Y}, \mu_\mathcal{Y})$, the Gromov--Wasserstein (GW) $p$-distance 
(for $p \geq 1$) between them is defined as
\begin{equation}
\label{eq:gw}
\mathrm{GW}_p(\mathcal{X}, \mathcal{Y})
=
\frac{1}{2}
\inf_{\pi \in \Pi(\mu_\mathcal{X}, \mu_\mathcal{Y})}
\left(
\iint_{(\mathcal{X}\times\mathcal{Y})^2}
\lvert
d_\mathcal{X}(x,x') - d_\mathcal{Y}(y,y')
\rvert^p
\,\mathrm{d}\pi(x,y)\,\mathrm{d}\pi(x',y')
\right)^{1/p}.
\end{equation}
A coupling $\pi$ can be interpreted as a probabilistic correspondence between the points
of $\mathcal{X}$ and $\mathcal{Y}$. The objective in \eqref{eq:gw} measures the expected
distortion of pairwise distances induced by this correspondence, and the optimization
seeks a coupling that minimizes the total discrepancy between the intrinsic metric
structures of the two spaces.

Let $\mathfrak{G}$ denote the collection of all metric measure spaces, i.e., $\mathfrak{G}
:=
\Big\{
(\mathcal{X}, d_\mathcal{X}, \mu_\mathcal{X})
\;\Big|\;
\text{mm-space}
\Big\}$, then $\mathcal{G}:= \mathfrak{G}/\cong$ is the space of all mm-spaces modulo measure-preserving isometries. The $\mathrm{GW}_p$ endows $\mathcal{G}$ with a metric structure by comparing the intrinsic geometries of mm-spaces through optimal transport.

\paragraph{Z-Gromov--Wasserstein.}
Following the general framework introduced by \cite{bauer2024z}, we consider \emph{$Z$-networks}, defined as triples $(\mathcal{X}, \omega_\mathcal{X}, \mu_\mathcal{X})$, where  $\omega_\mathcal{X} : \mathcal{X} \times \mathcal{X} \to \mathcal{Z}$
is a measurable function valued in a fixed metric space $(\mathcal{Z}, d_\mathcal{Z})$. The function $\omega_\mathcal{X}$ encodes pairwise relational information between points and is not required to arise from a metric.

Given two $Z$-networks $(\mathcal{X}, \omega_\mathcal{X}, \mu_\mathcal{X})$ and $(\mathcal{Y}, \omega_\mathcal{Y}, \mu_\mathcal{Y})$, the $Z$-Gromov--Wasserstein $p$-distance is defined as
\begin{equation}
\label{eq:zgw}
\mathrm{GW}^Z_p(\mathcal{X}, \mathcal{Y})
=
\frac{1}{2}
\inf_{\pi \in \Pi(\mu_\mathcal{X}, \mu_\mathcal{Y})}
\left(
\iint_{(\mathcal{X}\times\mathcal{Y})^2}
d_Z\!\left(
\omega_\mathcal{X}(x,x'),\,
\omega_\mathcal{Y}(y,y')
\right)^p
\,\mathrm{d}\pi(x,y)\,\mathrm{d}\pi(x',y')
\right)^{1/p}.
\end{equation}

More broadly, many GW variants used in machine learning can be interpreted as instances of $\mathrm{GW}^Z_p$ for suitable choices of the space $\mathcal{Z}$. When $\mathcal{Z}=\mathbb{R}$ endowed with the usual metric and $\omega_\mathcal{X}=d_\mathcal{X}$, $\omega_\mathcal{Y}=d_\mathcal{Y}$, the definition reduces to the $\mathrm{GW}_p$.


We denote by $\mathfrak{M}$ the collection of all $Z$-networks
$(\mathcal{X}, \omega_\mathcal{X}, \mu_\mathcal{X})$, and by
$\mathcal{M} := \mathfrak{M}/\cong$ the corresponding quotient space of
$Z$-networks modulo measure-preserving isomorphisms.

\paragraph{Working with representatives in practice.}
Although the quotient space $\mathcal{M} := \mathfrak{M}/\cong$ provides the
appropriate mathematical domain on which
$\mathrm{GW}^Z_p$-distances are well defined, it is not directly accessible in practice. Indeed, each element of $\mathcal{M}$ is an equivalence class containing multiple
isomorphic realizations, and any choice of a concrete representative in
$\mathfrak{M}$ is necessarily arbitrary. In practical settings, the observed data are therefore given as explicit
$Z$-networks in $\mathfrak{M}$ (i.e. Attributed Graphs, Graphs, Meshes, etc).
Since learning algorithms are trained on such concrete representations, their
outputs also naturally lie in $\mathfrak{M}$.
As a result, both prediction tasks and empirical datasets are necessarily
formulated at the level of $\mathfrak{M}$ rather than directly on the quotient
space $\mathcal{M}$.


\begin{definition}[Canonical Projection]
\label{def:can_proj}
The canonical projection $h : \mathfrak M \to \mathcal M$ is defined by $h(\tilde y) := [\tilde y]
= \{ \tilde y' \in \mathfrak M \mid \tilde y' \cong \tilde y \}.$ By construction, $h$ is surjective and generally many-to-one, and for any
$y \in \mathcal M$ one has $h^{-1}(y)\subseteq\mathfrak M$.
\end{definition}

\paragraph{Practical interpretation of the canonical projection.}
The canonical projection $h$ in Def.\ref{def:can_proj}  is not computed explicitly in practice.
Instead, quotienting is implemented implicitly through invariant comparison
operators.
In particular, the $\mathrm{GW}^Z_p$ defines a pseudometric on
$\mathfrak M$ that induces a metric on the quotient space $\mathcal M$.
In the ideal setting, this implies
\[
\mathrm{GW}^Z_p(\tilde y_1,\tilde y_2)=0
\quad \Longleftrightarrow \quad
h(\tilde y_1)=h(\tilde y_2),
\]
so that zero distance identifies representatives belonging to the same
equivalence class.

\subsection{Conformal Prediction with $Z$-networks}
In this section, we extend conformal prediction to a $Z$-network–valued output
setting. We assume the following.

\begin{assumption}[Representative-valued predictor]
We have access to a trained predictor $f_\theta : \mathcal X \to \mathfrak{M}$,
which maps an input $x \in \mathcal X$ to a concrete $Z$-network
$f_\theta(x) \in \mathfrak{M}$.
\end{assumption}

\begin{assumption}[Exchangeable data]
The observed data $(X_i,\tilde Y_i)_{i=1}^n$ are exchangeable and take values in
$\mathcal X \times \mathfrak M$.
\end{assumption}


Given a predictor $f_\theta$ and representative-valued data in $\mathfrak M$, we
define a nonconformity score
\[
\tilde s:\mathcal X\times\mathfrak M\to\mathbb R_+,
\qquad
\tilde s(x,\tilde y)
:= \mathrm{GW}^Z_p\!\big(f_\theta(x),\,\tilde y\big).
\]
Since $\tilde s$ is invariant under the equivalence relation $\cong$, it factors
through the canonical projection $h:\mathfrak M\to\mathcal M$ and induces a
well-defined score
\[
s:\mathcal X\times\mathcal M\to\mathbb R,
\qquad
s(x,y)=\tilde s(x,\tilde y),
\quad y=h(\tilde y),
\]
which depends only on the equivalence class of the output.

\begin{lemma}[Exchangeability is preserved under quotient maps]
\label{lem:exchangeability_preserved}
Let $(X_i,\tilde Y_i)_{i=1}^n$ be an exchangeable sequence of random variables
taking values in $\mathcal X \times \mathfrak M$.
Let $h:\mathfrak M\to\mathcal M:=\mathfrak M/\cong$ be the canonical projection
onto equivalence classes, and define $Y_i := h(\tilde Y_i)$.
Then the induced sequence $(X_i,Y_i)_{i=1}^n$ taking values in
$\mathcal X \times \mathcal M$ is exchangeable.
\end{lemma}

\begin{proof}
Exchangeability of $(X_i,\tilde Y_i)_{i=1}^n$ means that for any permutation
$\sigma$ of $\{1,\dots,n\}$,
\[
(X_1,\tilde Y_1,\dots,X_n,\tilde Y_n)
\;\overset{d}{=}\;
(X_{\sigma(1)},\tilde Y_{\sigma(1)},\dots,X_{\sigma(n)},\tilde Y_{\sigma(n)}).
\]

Define the measurable map $g:\mathcal X \times \mathfrak M \to \mathcal X \times \mathcal M$, 
$g(x,\tilde y) := (x,h(\tilde y))$.
Since $h$ is measurable, so is $g$.
Applying $g$ componentwise and invoking
Lemma~\ref{lem:measurable_preserve_law}, we obtain
\[
(X_1,Y_1,\dots,X_n,Y_n)
\;\overset{d}{=}\;
(X_{\sigma(1)},Y_{\sigma(1)},\dots,X_{\sigma(n)},Y_{\sigma(n)}),
\]
where $Y_i = h(\tilde Y_i)$.
Since this holds for all permutations $\sigma$, the sequence
$(X_i,Y_i)_{i=1}^n$ is exchangeable.
\end{proof}

Lemma~\ref{lem:exchangeability_preserved} ensures that the exchangeability of the
observed data is preserved when passing from representative-valued outputs in
$\mathfrak M$ to their equivalence classes in the quotient space $\mathcal M$.
However, conformal prediction is implemented by evaluating nonconformity scores
on concrete representatives in $\mathfrak M$.
Lemma \ref{lem:invariant_scores_exchangeable} shows that, provided the score is invariant under $\cong$,
representative-level evaluation induces an exchangeable score sequence that is
consistent with the exchangeability structure on $\mathcal M$.

\begin{lemma}[Invariant scores induce exchangeable sequences]
\label{lem:invariant_scores_exchangeable}
Let $(X_i,\tilde Y_i)_{i=1}^n$ be exchangeable random variables taking values in
$\mathcal X\times\mathfrak M$.
Let $\tilde s:\mathcal X\times\mathfrak M\to\mathbb R$ be a measurable
nonconformity score that is invariant under $\cong$.
Then the score sequence $S_i := \tilde s(X_i,\tilde Y_i), \;i=1,\dots,n,$
is exchangeable.
\end{lemma}
\begin{proof}
Since $\tilde s$ is invariant under $\cong$, it is constant on equivalence
classes of $\mathfrak M$ and therefore factors through the quotient map $h$.
Hence there exists a measurable function
$s:\mathcal X\times\mathcal M\to\mathbb R$ such that
\[
\tilde s = s \circ (\mathrm{id}_{\mathcal X}\times h),
\qquad
\tilde s(x,\tilde y)=s(x,h(\tilde y)).
\]
Define $Y_i:=h(\tilde Y_i)$.
By Lemma~\ref{lem:exchangeability_preserved}, the sequence $(X_i,Y_i)_{i=1}^n$
is exchangeable.
For any permutation $\sigma$ of $\{1,\dots,n\}$,
\[
(X_1,Y_1,\dots,X_n,Y_n)
\;\overset{d}{=}\;
(X_{\sigma(1)},Y_{\sigma(1)},\dots,X_{\sigma(n)},Y_{\sigma(n)}).
\]
Applying the measurable map $s$ componentwise and using
Lemma~\ref{lem:measurable_preserve_law}$,$
\[
\bigl(s(X_1,Y_1),\dots,s(X_n,Y_n)\bigr)
\;\overset{d}{=}\;
\bigl(s(X_{\sigma(1)},Y_{\sigma(1)}),\dots,s(X_{\sigma(n)},Y_{\sigma(n)})\bigr).
\]
Since $s(X_i,Y_i)=\tilde s(X_i,\tilde Y_i)$ for all $i$, the score sequence
$\{\tilde s(X_i,\tilde Y_i)\}_{i=1}^n$ is exchangeable.
\end{proof}

We now combine exchangeability preservation and score invariance to establish
conformal validity for $Z$-Gromov--Wasserstein–based prediction sets.

\begin{proposition}[Conformal validity on $\mathfrak M$ and $\mathcal M$]
\label{prop:conformal_validity_quotient}
Let $(X_i,\tilde Y_i)_{i=1}^n$ be exchangeable random variables taking values in
$\mathcal X\times\mathfrak M$, and let $f_\theta:\mathcal X\to\mathfrak M$ be a
predictor.
Define the nonconformity score
\[
\tilde s(x,\tilde y)
:= \mathrm{GW}^Z_p\!\big(f_\theta(x),\,\tilde y\big),
\]
and construct the conformal prediction set
$C^{\mathfrak M}_\alpha(x)\subseteq\mathfrak M$ at level $\alpha\in(0,1)$ using
$\tilde s$.
Then the following hold:
\begin{enumerate}
\item (\emph{Marginal coverage})
\[
\mathbb P\!\left(\tilde Y_{n+1}\in C^{\mathfrak M}_\alpha(X_{n+1})\right)\;\ge\;1-\alpha.
\]
\item (\emph{Well-defined on Quotient})
$C^{\mathfrak M}_\alpha(x)$ is a union of equivalence classes and therefore induces
a well-defined prediction set on the quotient space,
\[
C^{\mathcal M}_\alpha(x)
:= h\!\left(C^{\mathfrak M}_\alpha(x)\right)\subseteq\mathcal M,
\]
which satisfies
\[
\mathbb P\!\left(h(\tilde Y_{n+1})\in C^{\mathcal M}_\alpha(X_{n+1})\right)\;\ge\;1-\alpha.
\]
\end{enumerate}
\end{proposition}
\begin{proof}
By invariance of $\tilde s$ under $\cong$, it factors through the canonical
projection $h$ and induces a score on $\mathcal M$.
By Lemmas~\ref{lem:exchangeability_preserved} and
\ref{lem:invariant_scores_exchangeable}, the score sequence
$\{\tilde s(X_i,\tilde Y_i)\}_{i=1}^n$ is exchangeable.
Standard conformal prediction theory \cite{angelopoulos2023conformal} then yields
\[
\mathbb P\!\left(\tilde Y_{n+1}\in C^{\mathfrak M}_\alpha(X_{n+1})\right)\ge 1-\alpha.
\]
Since $\tilde s(x,\tilde y)=s(x,h(\tilde y))$, membership in
$C^{\mathfrak M}_\alpha(x)$ depends only on the equivalence class
$h(\tilde y)$.
Hence, for any $\tilde y,\tilde y'\in\mathfrak M$ with
$h(\tilde y)=h(\tilde y')$,
\[
\tilde y\in C^{\mathfrak M}_\alpha(x)
\quad\Longleftrightarrow\quad
\tilde y'\in C^{\mathfrak M}_\alpha(x),
\]
so $C^{\mathfrak M}_\alpha(x)$ is a union of equivalence classes.
Therefore the projection
\[
C^{\mathcal M}_\alpha(x):=h\!\left(C^{\mathfrak M}_\alpha(x)\right)
\]
is well defined. 
Let $Y_{n+1}:=h(\tilde Y_{n+1})$ denote the pushforward random variable, whose law
is the pushforward measure $P_{Y_{n+1}}=h_\# P_{\tilde Y_{n+1}}$.
Then
\[
\mathbb P\!\left(Y_{n+1}\in C^{\mathcal M}_\alpha(X_{n+1})\right)
=
\mathbb P\!\left(\tilde Y_{n+1}\in h^{-1}\!\left(C^{\mathcal M}_\alpha(X_{n+1})\right)\right)
=
\mathbb P\!\left(\tilde Y_{n+1}\in C^{\mathfrak M}_\alpha(X_{n+1})\right),
\]
where the second equality follows from the fact that
$h^{-1}(C^{\mathcal M}_\alpha(x))=C^{\mathfrak M}_\alpha(x)$.
Combining with the conformal coverage guarantee in $\mathfrak M$ yields
\[
\mathbb P\!\left(Y_{n+1}\in C^{\mathcal M}_\alpha(X_{n+1})\right)\ge 1-\alpha.
\]
\end{proof}

\GM{\textbf{Idea for figure schema} COMPUTE IN $\mathfrak{M}$, REASON IN $\mathcal{M}$, COVERAGE GUARANTEE IN BOTH}














==> source/useful_measure.tex <==
\section{Useful Math Results}
\begin{lemma}[Measurable maps preserve equality in distribution]
\label{lem:measurable_preserve_law}
Let $(\Omega,\mathcal F,\mathbb P)$ be a probability space.
Let $Z$ and $Z'$ be random variables taking values in a measurable space
$(\mathcal Z,\Sigma_{\mathcal Z})$, and let
$g : \mathcal Z \to \mathcal Y$ be a measurable map into another measurable space
$(\mathcal Y,\Sigma_{\mathcal Y})$.
If
\[
Z \overset{d}{=} Z',
\]
then
\[
g(Z) \overset{d}{=} g(Z').
\]
\end{lemma}

\begin{proof} Let $B \in \Sigma_{\mathcal Y}$ be arbitrary.
Since $g$ is measurable, $g^{-1}(B) \in \Sigma_{\mathcal Z}$, and therefore
\[
\mathbb P\big(g(Z) \in B\big)
= \mathbb P\big(Z \in g^{-1}(B)\big)
= \mathbb P\big(Z' \in g^{-1}(B)\big)
= \mathbb P\big(g(Z') \in B\big).
\]
Since this holds for all measurable sets $B \subseteq \mathcal Y$, we conclude that
$g(Z)$ and $g(Z')$ have the same distribution.
\end{proof}

